The Completed SDSS-IV extended Baryon Oscillation Spectroscopic Survey: Baryon acoustic oscillations with Lyman-$\alpha$ forests

We present a measurement of baryonic acoustic oscillations (BAO) from Lyman-$\alpha$ (Ly$\alpha$) absorption and quasars at an effective redshift $z=2.33$ using the complete extended Baryonic Oscillation Spectroscopic Survey (eBOSS). The sixteenth and final eBOSS data release (SDSS DR16) contains all data from eBOSS and its predecessor, the Baryonic Oscillation Spectroscopic Survey (BOSS), providing $210,005$ quasars with $z_{q}>2.10$ that are used to measure Ly$\alpha$ absorption. We measure the BAO scale both in the auto-correlation of Ly$\alpha$ absorption and in its cross correlation with $341,468$ quasars with redshift $z_{q}>1.77$. Apart from the statistical gain from new quasars and deeper observations, the main improvements over previous work come from more accurate modeling of physical and instrumental correlations and the use of new sets of mock data. Combining the BAO measurement from the auto- and cross-correlation yields the constraints of the two ratios $D_{H}(z=2.33)/r_{d} = 8.99 \pm 0.19$ and $D_{M}(z=2.33)/r_{d} = 37.5 \pm 1.1$, where the error bars are statistical. These results are within $1.5\sigma$ of the prediction of the flat-$\Lambda$CDM cosmology of Planck~(2016). The analysis code, \texttt{picca}, the catalog of the flux-transmission field measurements, and the $\Delta \chi^{2}$ surfaces are publicly available.

==> comments.tex <==
 De : RAVOUX Corentin
> Envoyé : lundi 15 juin 2020 16:35
> À : Rich James
> Objet : Article Lya eBOSS
>
> Salut Jim,
>
> je n'ai pas mis mon nom sur l'article auto-cross lyman-alpha. Est-ce que
> tu penses qu'il faut que je le mette ? (Peut-être dans la version
> corrigée) ou c'est trop tard ?
>
> Bonne soirée,
>
>
> Corentin
>



Plus haut dans le text, c’est (lambda_met - lambda_lya) / lambda_lya

Thomas

> On May 27, 2020, at 3:29 PM, Rich James <james.rich@cea.fr> wrote:
> 
> Oui, il manque qqchose, merci.  Mais c'est peutetre \lambda_{obs}?
> Jim
> ________________________________________
> De : Thomas Etourneau [thomas.etourneau@u-psud.fr]
> Envoyé : mercredi 27 mai 2020 15:23
> À : Rich James
> Objet : typo
> 
> Jim,
> 
> je viens de voir une typo dans le papier DR16 :
> dans le caption de la table 3, il manque le subscript Lya au dernier lambda dans la définition de rpar.
> 
> Thomas
> 




I've finally read the paper to catch up on the work done since DR12. 
It's a really nice and easy to read paper, good job.  
I have some questions/comments below.
Thanks

Julian

Intro:
- second to last paragraph: the two LRG papers are Bautista et al. 2020 and Gil-Marin et al. 2020

***  ok

- what do you mean by "this mask produces less data" in the last par. of 2.3?

*** It says ``This mask produces less data loss''  i.e. we mask fewer
pixels than the masks used in dr14,12...


Redshifts: 
- in sec 2.2. you say you use Z_LYAWG but in sec 3.1 you say you use Z_PCA. Which one do you use?

***  Z_LYAWG.  Will correct the mistatke, thanks

Section 4.5: 
- "Apart from improving the fit to the data, this procedure is necessary because the DR16 analysis combines all measurements of each quasar so spectra no longer correspond to a unique spectrograph". What are the 'measurements' here? Are you talking about the repeated observations?

***  yes, the repeated observations

- Why do you use MgII(11) band [260, 276] nm instead of the "calibration spectral region" [290, 312] nm for the sky correlations?  


***  That's Helion who did that--Don't know why

- "This test shows that the effect of the sky-subtractions residuals is mainly along the line-of-sight but a non negligible fraction is brought to other bins by the effects of continuum fitting.". Isn't the effect *transverse* to the line-of-sight, r_para = 0?

**** You're right.  Will change that


- Don't the same lambda correlations also arise from flux calibration errors, in addition to sky subtraction? c.f. section 5.2 of Bautista et al. 2017. Why are the calibration errors not mentioned any longer? 

**** Bautista et al concluded that the effect of the calibration vectors
was ``small''.  We wanted to repeat this test here but we didn't have
the time.


Figure 10: I would shift the transmission curve down to not overlap with the flux (black curve). Also, there are two DLA's in the Lya forest but just one is shown by a vertical dashed line. Is that intentional?

*** This is Helion's figure and it's hard to get him to change anything.
For the 2nd DLA, I'm not sure it was detected--I'll ask Helion


Sec 5.4: what prevented you from running the DLA finder on all mocks? 

****  A bug that slowed down considerably the finder.  We could do it now.

Sec 6.1: I don't understand the explanation that A_sky is one magnitude larger because of the 'effective redshift of the correlation functions'. In my mind sky residuals only depend on the observer frame wavelength and not if we are looking at Lyman-alpha or MgII forest.

**** I don't understand it either.  I'm not sure I would  have done
the study this way but that's Helion's baby.

Table 11: The reduction in chi2 is not negligible when adding BB terms. Have you looked at how typical is this reduction in mocks? It's all good for BAO but this would point to some effect that is not modelled correctly which would be interesting for full-shape analyses.

****  No, we never studied the BB with the mocks.  Yes, there's lots of
work to do here.  We certainly don't know what's going on here.











